Online Mobile App Usage as an Indicator of Sleep Behavior and Job Performance

Sleep is critical to human function, mediating factors like memory, mood, energy, and alertness; therefore, it is commonly conjectured that a good night's sleep is important for job performance. However, both real-world sleep behavior and job performance are hard to measure at scale. In this work, we show that people's everyday interactions with online mobile apps can reveal insights into their job performance in real-world contexts. We present an observational study in which we objectively tracked the sleep behavior and job performance of salespeople (N = 15) and athletes (N = 19) for 18 months, using a mattress sensor and online mobile app. We first demonstrate that cumulative sleep measures are correlated with job performance metrics, showing that an hour of daily sleep loss for a week was associated with a 9.0% and 9.5% reduction in performance of salespeople and athletes, respectively. We then examine the utility of online app interaction time as a passively collectible and scalable performance indicator. We show that app interaction time is correlated with the performance of the athletes, but not the salespeople. To support that our app-based performance indicator captures meaningful variation in psychomotor function and is robust against potential confounds, we conducted a second study to evaluate the relationship between sleep behavior and app interaction time in a cohort of 274 participants. Using a generalized additive model to control for per-participant random effects, we demonstrate that participants who lost one hour of daily sleep for a week exhibited 5.0% slower app interaction times. We also find that app interaction time exhibits meaningful chronobiologically consistent correlations with sleep history, time awake, and circadian rhythms. Our findings reveal an opportunity for online app developers to generate new insights regarding cognition and productivity.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)

==> chapters/corr-table.tex <==
% ========================================
% ========================================


% % spearman correlations

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{| *7{>{\centering\arraybackslash}m{1.2in}|} @{}m{0pt}@{}}
\multicolumn{1}{l}{}                               &\multicolumn{1}{l}{}                                                                                                 & \multicolumn{1}{l|}{}                & \multicolumn{4}{c|}{\textbf{Performance Metric}} & \rule{0pt}{0.5cm} \\ \cline{4-7}
\multicolumn{1}{l}{}                               &\multicolumn{1}{l}{}                                                                                                 & \multicolumn{1}{l|}{}               & \multicolumn{1}{c|}{\textbf{Athletics}}      & \multicolumn{2}{c|}{\textbf{Corporate Sales}}                                                                                & \textbf{App Interaction} \rule{0pt}{0.5cm}                                                      \\ 
\multicolumn{1}{l}{}                               &\multicolumn{1}{l}{}                                                                                                 & \multicolumn{1}{l|}{}               & \multicolumn{1}{c|}{Game Grades}             & Hires                               & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Attorney Fees\\ Collected\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Interaction Speed\\ (smaller = better)\end{tabular} \\ \hline
\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{}                                                               & \multicolumn{1}{c|}{Total Duration} & \multicolumn{1}{c|}{0.0176 (0.818)}          & \multicolumn{1}{c|}{-0.0453 (0.625)} & \multicolumn{1}{c|}{-0.0635 (0.493)}                                                   & -0.014 (0.0661) & \rule{0pt}{0.75cm}      \\

\multicolumn{1}{c|}{}                              &\multicolumn{1}{c|}{}                                                                                                & \multicolumn{1}{c|}{Sleep Debt}     & \multicolumn{1}{c|}{-0.0680 (0.374)}         & \textbf{0.206 (0.0291)}             & \multicolumn{1}{c|}{0.0376 (0.694)}                                                    & \textbf{-0.0973 (6.06e-33)} & \rule{0pt}{0.75cm}                                                   \\ 
\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{\rotatebox{90}{\rlap{\tabular{@{}c}Raw Metric\endtabular}}}                                                                                                                             & \multicolumn{1}{c|}{Sleep History}  & \multicolumn{1}{c|}{-0.0599 (0.428)}         & 0.0607 (0.535)                      & \multicolumn{1}{c|}{-0.00316 (0.974)}                                                  & \textbf{-0.0544 (2.18e-11)}  & \rule{0pt}{0.75cm}                                                  \\
\cline{2-7}
\multicolumn{1}{c|}{\rotatebox{90}{\rlap{\tabular{@{}c} \textbf{Sleep Metric}\endtabular}}}                              &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Total Duration} & \multicolumn{1}{c|}{0.116 (0.129)}           & -0.126 (0.173)                      & \multicolumn{1}{c|}{-0.0905 (0.328)}                                                   & 0.00533 (0.486) & \rule{0pt}{1.2cm}                                                               \\
\multicolumn{1}{c|}{}                              &\multicolumn{1}{c|}{\rotatebox{90}{\rlap{\tabular{@{}c}Per-person \\ Z-normalized Metric\endtabular}}}                                                                                                & \multicolumn{1}{c|}{Sleep Debt}     & \multicolumn{1}{c|}{\textbf{0.174 (0.0221)}} & 0.182 (0.0565)                      & \multicolumn{1}{c|}{-0.00652 (0.946)}                                                  & -0.00953 (0.243)  \\

\multicolumn{1}{c|}{}                              &\multicolumn{1}{c|}{}                                                                                                & \multicolumn{1}{c|}{Sleep History}  & \multicolumn{1}{c|}{\textbf{0.158 (0.0362)}} & -0.0186 (0.851)                     & \multicolumn{1}{c|}{-0.0405 (0.682)}                                                   & -0.0132 (0.105) & \rule{0pt}{1.2cm}                                                               & \rule{0pt}{1.2cm} \\ \hline                                        
\end{tabular}%
}
\caption{Spearman correlations, p-values in parentheses. Results with p-value < 0.05 shown in bold.}
\label{tab:spearman-corr-transpose}
\end{table}

% ========================================
% ========================================


% % spearman correlations, no sleep debt.
% \begin{table}[tb] %hp
%     \centering
%     % \begin{tabular}{ccccc}
%     \hspace*{-2cm}
%     \begin{tabular}{c|cc|cc}
%     & \multicolumn{2}{c|}{ \textbf{Raw Sleep Data} } & 
%     % \multicolumn{2}{c}{ \textbf{\ \ Per Person Z-Normalization of Sleep Data\ \ } } \\
%     \multicolumn{2}{c}{ \textbf{\ \ Individualized Z-Normalization\ \ } } \\
%     % Dataset & 
%     % \parbox[b]{\corrTableColOneWidth\linewidth}{\centering Performance Metric} & Total Duration & Sleep History & Total Duration & Sleep History \\
%     \parbox[b]{\corrTableColOneWidth\linewidth}{\centering Performance Metric} & 
%     \parbox[b]{\corrTableColWidth\linewidth}{\centering Total Duration} & 
%     \parbox[b]{\corrTableColWidth\linewidth}{\centering Sleep History} & 
%     \parbox[b]{\corrTableColWidth\linewidth}{\centering Total Duration} & 
%     \parbox[b]{\corrTableColWidth\linewidth}{\centering Sleep History} \\
%     \hline
    
%     % \multirow{2}{*}{ Performance Metric } & \multicolumn{2}{c}{ Raw Sleep Data } & \multicolumn{2}{c}{ Per Person Z-Normalization of Sleep Data } \\
%     % & Total Duration & Sleep History & Total Duration & Sleep History \\
    
%     \textbf{Athletics} & & & & \\
%     Game Grade & -0.0272 (0.873) & -0.0599 (0.428) & & \textbf{0.158 (0.0362)} \\
%     \hline
    
%     \textbf{Corporate Sales} & & & & \\
%     Hires & -0.0453 (0.625) & 0.0607 (0.535) & -0.126 (0.173) & -0.0186 (0.851) \\
%     Attorney Fees Collected & -0.0635 (0.493) & -0.00316 (0.974) & -0.0905 (0.328) & -0.0405 (0.682) \\
%     Number of Calls & -0.0548 (0.364) & 0.0893 (0.168) & -0.22 (0.00023) & -0.252 (8.49e-05) \\
%     \hline
    
%     \textbf{Mobile App} & & & & \\
%     \parbox[c]{\corrTableColOneWidth\linewidth}{\centering Interaction Speed (smaller = better)} & -0.014 (0.0661) & \textbf{-0.0544 (2.18e-11)} & 0.00533 (0.486) & -0.0132 (0.105) \\
    
%     \end{tabular}
%     \hspace*{-2cm}
    
%     \caption{Spearman correlations, p-values in parentheses. Results with p-value < 0.05 shown in bold.}
%     \label{tab:spearman-corr}

% \end{table}

==> chapters/old-corr-table-job-perf.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[tbh]
\centering
%\resizebox{\textwidth}{!}{%
\begin{tabular}{| *6{>{\centering\arraybackslash}m{1.2in}} @{}m{0pt}@{}}
\cline{4-6}
\multicolumn{1}{l}{} &\multicolumn{1}{l}{} & \multicolumn{1}{l|}{}                & \multicolumn{3}{c|}{\textbf{Job Performance Metric}} & \rule{0pt}{0.5cm} \\ \cline{4-6}
\multicolumn{1}{l}{}                               &\multicolumn{1}{l}{}                                                                                                 & \multicolumn{1}{l|}{}               & \multicolumn{1}{c|}{\textbf{NFL Players}}      & \multicolumn{2}{c|}{\textbf{Call Center Employees}}                                                                                & \rule{0pt}{0.5cm}                                                      \\ 


% total_duration
% \multicolumn{1}{c|}{-0.0244 ($p$=0.751)} & -0.0453 ($p$=0.6248) & \multicolumn{1}{c|}{-0.0635 ($p$=0.4929)} & \rule{0pt}{0.75cm} \\ 
% sleep_debt2
% \multicolumn{1}{c|}{-0.0285 ($p$=0.711)} & 0.0607 ($p$=0.5346) & \multicolumn{1}{c|}{-0.0032 ($p$=0.9742)} & \rule{0pt}{0.75cm} \\ 
% sleep_debt
% \multicolumn{1}{c|}{-0.0949 ($p$=0.2183)} & \textbf{0.2063 ($p$=0.0291)} & \multicolumn{1}{c|}{0.0376 ($p$=0.6939)} & \rule{0pt}{0.75cm} \\ 

% total_duration_Z
% \multicolumn{1}{c|}{0.086 ($p$=0.2632)} & -0.1258 ($p$=0.1728) & \multicolumn{1}{c|}{-0.0905 ($p$=0.3279)} & \rule{0pt}{0.75cm} \\ 
% sleep_debt2_Z
% \multicolumn{1}{c|}{\textbf{0.1785 ($p$=0.0195)}} & -0.0225 ($p$=0.8194) & \multicolumn{1}{c|}{-0.0297 ($p$=0.7639)} & \rule{0pt}{0.75cm} \\ 
% sleep_debt_Z
% \multicolumn{1}{c|}{\textbf{0.1659 ($p$=0.0307)}} & 0.163 ($p$=0.0888) & \multicolumn{1}{c|}{-0.0281 ($p$=0.7708)} & \rule{0pt}{0.75cm} \\ 


\multicolumn{1}{l}{}                               &\multicolumn{1}{l}{}                                                                                                 & \multicolumn{1}{l|}{}               & \multicolumn{1}{c|}{Game Grades}             & Hires                               & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Attorney Fees\\ Collected\end{tabular}} \\ \hline

% % start hour, end hour, midpoint rows begin here.

% \multicolumn{1}{c|}{} &\multicolumn{1}{c|}{}                                                               & \multicolumn{1}{c|}{Start Time} & 
% \multicolumn{1}{c|}{-0.0476 ($p$=0.5365)} & 0.0866 ($p$=0.3491) & \multicolumn{1}{c|}{0.0132 ($p$=0.8869)} & \rule{0pt}{0.75cm} \\ 

% \multicolumn{1}{c|}{} &\multicolumn{1}{c|}{}                                                               & \multicolumn{1}{c|}{End Time} & 
% \multicolumn{1}{c|}{-0.0624 ($p$=0.4177)} & 0.063 ($p$=0.4958) & \multicolumn{1}{c|}{-0.0654 ($p$=0.4801)} & \rule{0pt}{0.75cm} \\ 

% \multicolumn{1}{c|}{} &\multicolumn{1}{c|}{}                                                               & \multicolumn{1}{c|}{Midpoint} & 
% \multicolumn{1}{c|}{-0.0869 ($p$=0.2582)} & 0.1644 ($p$=0.0741) & \multicolumn{1}{c|}{0.0127 ($p$=0.8912)} & \rule{0pt}{0.75cm} \\ 

% total duration, sleep history, sleep debt rows start here.

\multicolumn{1}{|c|}{} &\multicolumn{1}{c|}{}                                                               & \multicolumn{1}{c|}{Total Duration} & 
% \multicolumn{1}{c|}{0.0176 ($p$=0.818)}          & \multicolumn{1}{c|}{-0.0453 ($p$=0.625)} & \multicolumn{1}{c|}{-0.0635 ($p$=0.493)}                                                   & \rule{0pt}{0.75cm}      \\
\multicolumn{1}{c|}{-0.0244 ($p$=0.751)} & -0.0673 ($p$=0.469) & \multicolumn{1}{c|}{-0.0864 ($p$=0.352)} & \rule{0pt}{0.75cm} \\ 

\multicolumn{1}{|c|}{}                              &\multicolumn{1}{c|}{}                                                                                                & \multicolumn{1}{c|}{Sleep History}  & 
% \multicolumn{1}{c|}{-0.0599 ($p$=0.428)}         & 0.0607 ($p$=0.535)                      & \multicolumn{1}{c|}{-0.00316 ($p$=0.974)}                                                  & \rule{0pt}{0.75cm}                                                  \\
\multicolumn{1}{c|}{-0.0285 ($p$=0.711)} & 0.0392 ($p$=0.6901) & \multicolumn{1}{c|}{-0.0278 ($p$=0.7773)} & \rule{0pt}{0.75cm} \\ 


\multicolumn{1}{|c|}{}                              &\multicolumn{1}{c|}{\rotatebox{90}{\rlap{\tabular{@{}c}\hspace{0.15cm}Raw Metric\endtabular}}}                                                                                                & \multicolumn{1}{c|}{Sleep Debt}     & 
% \multicolumn{1}{c|}{-0.0680 ($p$=0.374)}         & \textbf{0.206 ($p$=0.0291)}             & \multicolumn{1}{c|}{0.0376 ($p$=0.694)}                                                    & \rule{0pt}{0.75cm}                                                   \\ 
\multicolumn{1}{c|}{-0.0949 ($p$=0.2183)} & \textbf{0.2181 ($p$=0.0215)} & \multicolumn{1}{c|}{0.046 ($p$=0.6318)} & \rule{0pt}{0.75cm} \\ 
\cline{2-6}

% % start hour, end hour, midpoint z-norm rows start here.

% \multicolumn{1}{c|}{}                              &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Start Time} &
% \multicolumn{1}{c|}{0.0032 ($p$=0.9665)} & 0.1517 ($p$=0.1086) & \multicolumn{1}{c|}{0.1041 ($p$=0.2726)} & \rule{0pt}{0.75cm} \\ 

% \multicolumn{1}{c|}{}                              &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{End Time} &
% \multicolumn{1}{c|}{-0.021 ($p$=0.7851)} & 0.0277 ($p$=0.7708) & \multicolumn{1}{c|}{-0.052 ($p$=0.5844)} & \rule{0pt}{0.75cm} \\ 

% \multicolumn{1}{c|}{}                              &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Midpoint} &
% \multicolumn{1}{c|}{-0.0529 ($p$=0.4918)} & 0.1717 ($p$=0.069) & \multicolumn{1}{c|}{0.0632 ($p$=0.5059)} & \rule{0pt}{0.75cm} \\ 

% total duration, sleep history, sleep debt z-norm rows start here.

\multicolumn{1}{|c|}{}                              &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Total Duration} &
% \multicolumn{1}{c|}{0.116 ($p$=0.129)}           & -0.126 ($p$=0.173)                      & \multicolumn{1}{c|}{-0.0905 ($p$=0.328)}                                                   & \rule{0pt}{0.75cm}                                                               \\
\multicolumn{1}{c|}{0.086 ($p$=0.2632)} & -0.1023 ($p$=0.283) & \multicolumn{1}{c|}{-0.1012 ($p$=0.2886)} & \rule{0pt}{0.75cm} \\ 

\multicolumn{1}{|c|}{\rotatebox{90}{\rlap{\tabular{@{}c} \textbf{\hspace{0.5cm}Sleep Metric}\endtabular}}}                              &\multicolumn{1}{c|}{}                                                                                                & \multicolumn{1}{c|}{Sleep History}  &
\multicolumn{1}{c|}{\textbf{0.1785 ($p$=0.0195)}} & -0.0473 ($p$=0.6337) & \multicolumn{1}{c|}{-0.0556 ($p$=0.5753)} & \rule{0pt}{0.75cm} \\ 

% \multicolumn{1}{c|}{\textbf{0.158 ($p$=0.0362)}} & -0.0186 ($p$=0.851)                     & \multicolumn{1}{c|}{-0.0405 ($p$=0.682)}                                                   & \rule{0pt}{0.75cm}                                                               \\
\multicolumn{1}{|c|}{}                              &\multicolumn{1}{c|}{\rotatebox{90}{\rlap{\tabular{@{}c}Per-person \\ Z-normalized \\ Metric\endtabular}}}                                                                                                & \multicolumn{1}{c|}{Sleep Debt}     &
\multicolumn{1}{c|}{\textbf{0.1659 ($p$=0.0307)}} & 0.1642 ($p$=0.0879) & \multicolumn{1}{c|}{-0.0294 ($p$=0.7618)} & \rule{0pt}{0.75cm} \\ 

\hline
% \multicolumn{1}{c|}{\textbf{0.174 ($p$=0.0221)}} & 0.182 ($p$=0.0565)                      & \multicolumn{1}{c|}{-0.00652 ($p$=0.946)}                                                  & \rule{0pt}{0.75cm} \\ \hline                                        
\end{tabular}%
%}
\caption{Spearman correlation coefficients between sleep behavior and job performance. P-values are provided in parentheses; results with p-value < 0.05 are shown in bold.}
\label{tab:spearman-corr-job-perf}
\end{table}



==> chapters/old-corr-table-job-performance.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\begin{tabular}{| *6{>{\centering\arraybackslash}m{1.2in}} @{}m{0pt}@{}}
\cline{4-6}
\multicolumn{1}{l}{} &\multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{3}{c|}{\textbf{Job Performance Metric}} & \rule{0pt}{0.5cm} \\ \cline{4-6}
\multicolumn{1}{l}{} &\multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{NFL Players} \\ \revision{\textbf{($N=19$)}}\end{tabular}}      & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Call Center Employees} \\ \revision{\textbf{($N=15$)}}\end{tabular}}                                                                                & \rule{0pt}{0.5cm}                                                      \\ 

\multicolumn{1}{l}{}                               &\multicolumn{1}{l}{}                                                                                                 & \multicolumn{1}{l|}{}               & \multicolumn{1}{c|}{Game Grades}             & Hires                               & \multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Attorney Fees\\ Collected\end{tabular}} \\ \hline

\multicolumn{1}{|c|}{} &\multicolumn{1}{c|}{}                                                               & \multicolumn{1}{c|}{\revision{Time-in-Bed}} & 
\multicolumn{1}{c|}{-0.024 ($p$=0.751)} & -0.067 ($p$=0.469) & \multicolumn{1}{|c|}{-0.086 ($p$=0.352)} & \rule{0pt}{0.75cm} \\ 

\multicolumn{1}{|c|}{}                              &\multicolumn{1}{c|}{}                                                                                                & \multicolumn{1}{c|}{Sleep Debt}     & 
\multicolumn{1}{c|}{-0.095 ($p$=0.218)} & \textbf{0.218 ($p$=0.022)} & \multicolumn{1}{|c|}{0.046 ($p$=0.632)} & \rule{0pt}{0.75cm} \\

\multicolumn{1}{|c|}{}                              &\multicolumn{1}{c|}{\rotatebox{90}{\rlap{\tabular{@{}c}\hspace{0.15cm}Raw Metric\endtabular}}}                                                                                                & \multicolumn{1}{c|}{Sleep History}  & 
\multicolumn{1}{c|}{-0.029 ($p$=0.711)} & 0.039 ($p$=0.690) & \multicolumn{1}{|c|}{-0.028 ($p$=0.777)} & \rule{0pt}{0.75cm} \\ 

\cline{2-6}
\multicolumn{1}{|c|}{}                              &\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\revision{Time-in-Bed}} &
\multicolumn{1}{c|}{0.086 ($p$=0.263)} & -0.102 ($p$=0.283) & \multicolumn{1}{|c|}{-0.101 ($p$=0.289)} & \rule{0pt}{0.75cm} \\ 

\multicolumn{1}{|c|}{\rotatebox{90}{\rlap{\tabular{@{}c} \textbf{\hspace{0.5cm}Sleep Metric}\endtabular}}}  &\multicolumn{1}{c|}{}                                                                                               & \multicolumn{1}{c|}{Sleep Debt}     &
\multicolumn{1}{c|}{\textbf{0.166 ($p$=0.031)}} & 0.164 ($p$=0.088) & \multicolumn{1}{|c|}{-0.029 ($p$=0.762)} & \rule{0pt}{0.75cm} \\ 

\multicolumn{1}{|c|}{}                             &\multicolumn{1}{c|}{\rotatebox{90}{\rlap{\tabular{@{}c}Per-person \\ Z-normalized \\ Metric\endtabular}}}                                                                                                & \multicolumn{1}{c|}{Sleep History}  &
\multicolumn{1}{c|}{\textbf{0.179 ($p$=0.020)}} & -0.047 ($p$=0.634) & \multicolumn{1}{|c|}{-0.056 ($p$=0.575)} & \rule{0pt}{0.75cm} \\ 

\hline
\end{tabular}%

\end{table}

==> revisions/1ae.tex <==
\subsection{1AE} % major revision, significant impact
\label{sec:revisions-1ae}
We would like to thank the 1AE for concisely summarizing the reviewers' responses. We have repeated the most important changes here to address the topics covered in the meta-reivew, but many more details can be found in response to the specific reviewer comments.

\begin{enumerate}[labelsep=6mm,label=(1AE-\arabic*)]
\item \reviewcomment{Overclaims: The claims in the title and abstract seem somewhat misleading compared to the actual findings presented in the paper (R2, R4, R5). R5 noted ``finding out that N=15 and N=19 on Page 8 is really, really rough''. R3 also mentioned ``RQ1 and RQ3 are related to the subpopulation of athletes and salespeople which make up only 12\% of the 274 participants''. This inconsistency between abstract/title and later content is a major issue with the current article and it will be essential to address this issue for a successful revision. I recommend updating the title, abstract, and overall narrative to be consistent with the contributions of the paper.}
The reviewers raised important points on how we represented our data. We have made numerous changes throughout the revised article to be more clear about the sample sizes for each analysis. The sample sizes (i.e., number of users and number of data points) are explicitly mentioned in the following sections and tables:
\begin{itemize}[leftmargin=.35in]
    \item Abstract
    \item Section~\ref{sec:intro}: Introduction
    \item Section~\ref{sec:datasets-job}: Job Performance Metrics
    \item Table~\ref{tab:dataset}: Dataset summary statistics
    \item Section~\ref{sec:methods}: Research Questions and Methods
    \item Section~\ref{sec:results}: Results
    \item Table~\ref{tab:spearman-corr-job-perf}: Analysis for RQ.1
\end{itemize}
Additionally, we have changed the title to ``Sleep Behavior, Job Performance, and Their Indicators in Mobile App Usage''. This title does not mention the notion of athletes and salespeople in our dataset to avoid misleading readers into thinking that the entire dataset consists of those individuals, and it also gives equal weighting to the three components of our dataset. \\

\item \reviewcomment{Ground truth: There are also a number of questions regarding the validity of the data used in this paper. R2 noted that time in bed does not equal to sleep. They should also clarify points raised by R2 and R4 regarding the accuracy of mattress sensing in detecting sleep events. Using app interaction features as indicators of alertness or cognitive capacity requires more justification (R2, R5). It will also be important to address the questions regarding smartphone based sleep sensing as raised by R5.}
We thank the reviewers for requesting more justification for these data sources, and we also thank the 1AE for summarizing these issues. We have clarified some of these points and added more references to justify others. We provide a detailed response to each below: \\

\textbf{Time-in-bed $\neq$ sleep (2AE):} We agree that there is a nuance between ``time-in-bed'' and ``total sleep duration'' since people may not fall asleep as soon as they get into their bed. The Emfit QS mattress sensor reports both metrics, but we restricted our analyses to time-in-bed because it only requires accurate presence detection; total sleep duration requires accurate presence and sleep detection, thus adding an additional source of potential uncertainty. We have updated all mentions of total sleep duration to time-in-bed and updated the definition in Table~\ref{tab:metrics}. Literature has shown that time-in-bed recorded from sleep diaries is highly correlated with total sleep duration~\cite{Rogers1993}. We calculated the Pearson correlation between time-in-bed and total sleep duration in our dataset and also found a strong correlation ($\rho=0.85, p<.001$). Furthermore, we re-ran our analyses with total sleep duration instead of time-in-bed and found comparable correlations in almost all cases. We mention that we tested both metrics in Section~\ref{sec:dataset-sleep}. \\

\textbf{Accuracy of mattress sensor (2AE, R4, R5):} In our original article, we cited Ranta et al.~\cite{Ranta2019} as a reference that compared the Emfit QS sensor against polysomnography. They found ~98\% agreement between the two sensors in terms of heart rate and respiratory rate tracking. We have added two other references~\cite{Guerrero-Mora2012,Kortelainen2010} to our article that compared the Emfit QS sensor to polysomnography. Guerrero-Mora et al.~\cite{Guerrero-Mora2012} found that the Emfit QS sensor was 80\% accurate in detecting sleep/wake events when compared to expert annotations of polysomnography data. Kortelainen et al.~\cite{Kortelainen2010} further evaluated the Emfit QS sensor in regards to sleep stage classification against experts' annotation from polysomnography, again finding that the Emfit QS has 83\% sensitivity and specificity. R5 also had a question regarding partners who shared the same bed. The Emfit QS sensor comes with instructions that explain how to install the sensor in situations when a bed is shared by multiple people (page 6 of \cite{Emfit2018}). The sensor can be placed so that it lies solely on the user's preferred side of the bed. The sensor has been designed to filter out smaller displacements in favor of larger ones caused by the user lying directly on top of the sensor. We have added this information to the revised article. \\

\textbf{App interaction as an indicator of alertness (2AE, R5):}  To further motivate our use of mobile app usage as an indicator of cognition and performance, we have added additional examples of prior work in this space to Section~\ref{sec:related-interaction}~\cite{Mark2014,Pielot2015,Oulasvirta2012,Vizer2009,Mehrotra2016,Ferdous2015}. For example, Murnane et al.~\cite{Murnane2016} demonstrate that app usage patterns vary for individuals with different chronotypes and rhythms of alertness. Oulasvirta et al.~\cite{Oulasvirta2012} correlate frequent, short bursts of smartphone interaction with inattentiveness, and Vizer et al.~\cite{Vizer2009} used variation and drift in keystroke rate to infer stress. We assert that our findings in Section~\ref{sec:rq2} aligns with expectations from prior work, which gives credibility to the use of app interaction as an indicator of alertness. For example, our findings illustrate that users typically had slower interaction times immediately after waking up, which aligns with the chronobiological process of sleep inertia~\cite{Akerstedt1997}. We also found that interaction time decreased during the first six hours after wakeup and then increased again, which is consistent with the chronobiological process of homeostatic drive~\cite{Borbely2016}. \\

\textbf{Smartphone-based sensing (R5):} First, we would like to ensure that there is no confusion about the nature of our study. Sleep sensing was only performed by the mattress sensor; the app was strictly for viewing the sensor's data through a user-friendly interface. As for the use of a smartphone-based technique as a fallback for when participants did not carry their mattress sensor with them, this would be an excellent follow-up study for the UbiComp community. There have been numerous efforts in sleep sensing using technologies like smartphones and smartwatches~\cite{Ko2015,Min2014,Rahman2015,Byanna2016}, and they have achieved promising results. We actually investigated the inclusion of a sleep detection app that leveraged the accelerometer to sense bed motion. At the time, we found that the mobile app generally overestimated time-in-bed by 1-2 hours. These errors, combined with the burden of battery drain, led us to not feel comfortable with the introduction of an additional source of uncertainty. \\

\item \reviewcomment{Analysis and findings: R2 and R4 noted that the correlation analysis presented in the paper require more details. There is also confusion about which results correspond to which sub-populations (R4). R5 pointed out the potential issues related to compliance. R5 also provided a number of ideas for improving the analysis and findings (e.g., controlling for chronotypes, comparison between weekday and weekends, ...). Furthermore, R5 listed a number of potential concerns and confounding factors (e.g., variations across work hours, chronotypes, weekdays vs weekends, impact of naps and caffeine, travel and timezone shifts, ...). I encourage authors to address these concerns, if possible given the dataset.}
We thank the reviewers for pointing out places in our article that require additional clarity. We also appreciate the many insightful directions for future work. We address each of these topics below: \\

\textbf{More details for the correlation analysis (2AE, R4):} We believe that this is referring to the questions that these reviewers had about the significance of our analyses. Our original submission listed multiple effect sizes when our correlation coefficients were found to be significant. To address questions that multiple reviewers had about the significance of the effect sizes, we expanded some of them by converting percentages to absolute quantities. We have enumerated the effect sizes presented in the article below for your convenience (revisions to the article are in red):
\begin{itemize}[leftmargin=.35in]
    \item ``One hour of sleep loss the night before by the average salesperson resulted in 1.9\% decrease in the number of hires they were able to make. \revision{The average salesperson made 3.8 hires per workday and collected \$936 in fees per hire. Therefore, a 1.9\% decrease translates to a \$67 loss per day.}'' (Section~\ref{sec:rq1})
    \item ``The average athlete experienced a 2.0\% drop \revision{(1.3 points)} in their game grade when they lost one hour of sleep the night before.'' (Section~\ref{sec:rq1})
    \item ``A more severe, but not uncommon scenario of losing an hour of sleep every day for a week is equivalent to losing 4.75 hours of sleep yesterday or 11.2 hours of sleep one week ago. On average, this loss in sleep debt causes a 9.5\% \revision{(6.2 points)} reduction in game performance, and a 9\% \revision{(\$317)} reduction in hires for salespeople.'' (Section~\ref{sec:rq1})
    \item ``For one hour of sleep history improvement, the average athlete improved their game grade by 5.7\%.'' (Section~\ref{sec:rq1})
    \item ``Users who accumulated one less hour of sleep debt were 0.2 seconds faster each time they moved between app screens.'' (Section~\ref{sec:rq2})
    \item ``On average, interaction time increases by 0.4 seconds when sleep history improves from 6 to 8 hours, and interaction time increases by 0.5 seconds beyond the threshold of -5 sleep debt hours.'' (Section~\ref{sec:rq2})
    \item ``The effect size shows that athletes who were 10 seconds faster in their interaction time, on average had 5 more points higher game grades.'' (Section~\ref{sec:rq3})
    \item ``Participants who engaged with the app for 35 days on average slept 42 minutes longer, had 3.5 hours less sleep debt, and went to bed 48 minutes earlier, compared to less engaged users that opened the app on only 7 days. Participants who engaged with the app more often also exhibited more consistent bedtimes, with the standard deviation dropping from 1.4 hours to 1.2 hours.'' (Section~\ref{sec:rq4})
    \item ``Higher app engagement was consistently associated with an improvement in average time-in-bed within users, with an average increase in time-in-bed of about 15 minutes per night.'' (Section~\ref{sec:rq4})
\end{itemize}
Regarding the magnitude of the statistically significant results we presented, we posit that larger effect sizes are not necessarily expected in this setting. As a point of comparison, Althoff et al.~\cite{Althoff2017} found that hour-long differences in time-in-bed resulted in keystroke timing differences of a few milliseconds ($\sim$3.5\%). As R5 thoroughly comments in their review, the small performance impacts we see are partly due to the rich set of factors impacting sleep and performance. For instance, sleep behavior is known to be affected by ambient light~\cite{Kozaki2005}, caffeine intake~\cite{Landolt1995}, and diet~\cite{Halson2008}, while salesperson job performance is influenced by their on-job experience and the state of the economy. Still, we were able to uncover statistically significant results that aligned with expectations from sleep science~\cite{Akerstedt1997,Borbely2016,Dijk1992}. Therefore, we believe these findings are meaningful to the research community. \\

\textbf{Analysis for subpopulations vs. entire dataset (R4):} We have repeated our sample size numbers throughout the paper, including both Section~\ref{sec:methods} and Section~\ref{sec:results} where they are most convenient for readers. \\

\textbf{Compliance (R5):} The large standard deviations in Table~\ref{tab:dataset} implies to readers that compliance was low and lots of imputation was needed in our dataset. However, we believe that these numbers are a bit misleading in that regard. Compliance can be broken into two levels: organization engagement and participant compliance. Regarding organization engagement, our dataset is the product of a collaboration with multiple organizations. To recruit the NFL players, for example, we were unable to engage with the entire league and thus had to form partnerships with individual teams. Although our data collection period lasted 1.5 years, the level of engagement we had with different organizations varied. The bankruptcy law firm consultancy was enrolled for 225 days, and the NFL teams were enrolled from 457--518 days. Across our entire population, participants were enrolled for 83--578 days. This aspect of our recruitment means that even if participants engaged with the sleep-tracking technology every day, there would still be large variance in the number of nights of tracked sleep as summarized in Table~\ref{tab:dataset}. \\

Regarding participant compliance, participants were free to enroll and leave the study as they pleased. Participants were also free to use the sleep-tracking technology however they wanted. This was done to reduce friction with our partnered organizations and to generate the most natural data possible (in a free-living setting). Table~\ref{tab:imputed_sleep} shows the fraction of sleep duration values that were imputed in the calculation of the sleep history metric. 
A full week of sleep data was available for calculating 46.9\% of the cumulative sleep metrics, meaning that no imputation was needed for them. Three or more nights were only missing in 12.7\% of the cumulative sleep metrics. Thus, little imputation was necessary, even for the longer sleep history measures.
\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c}
         Number of & Full & & \\
         Imputed Days & Population & Salespeople & Athletes \\
         \hline
         0 & 46.9\% & 49.2\% & 29.2\% \\
         1 & 24.6\% & 15.3\% & 45.3\% \\
         2 & 15.8\% & 13.6\% & 12.3\% \\
         3 & 8.6\% & 16.1\% & 8.2\% \\
         4 & 4.1\% & 5.9\% & 5.0\% 
    \end{tabular}
    \caption{Number of imputed days in sleep history calculation.}
\end{table}
We agree with R5 that the matter of imputation and compliance should be highlighted much earlier in the paper. Our original article described the nature of our recruitment process in Section~\ref{sec:dataset-population} and our imputation procedure in Section~\ref{sec:dataset-sleep}. On top of this, we have removed the ``Observation Period'' row in Table~\ref{tab:dataset} to avoid misleading readers into thinking that enrollment was continuous. We provide the above reasoning in Section~\ref{sec:datasets-filtering} to describe why the standard deviations are so large in Table~\ref{tab:dataset}. We have also added statistics on the amount of imputation that was needed in Section~\ref{sec:datasets-filtering}.\\

\textbf{Confounds and controlling factors (R5):} R5 listed many insightful comments about possible confounds in our dataset. We have addressed each and every one of R5's suggestions in their portion of this response document, but space precludes us from repeating all of them here. In short, we share R5's excitement about many of the dynamics that drive sleep and performance. We have been able to address some of these in our analysis:
\begin{itemize}[leftmargin=.35in]
    \item \textbf{Naps:} The time-in-bed metric we report includes naps that were either automatically tagged by the Emfit QS or manually annotated post-hoc by the user if they were missed. We feel that it is important to include naps in our dataset because naps contribute to sleep recovery and therefore play a role in sleep debt/sleep history~\cite{Matsumoto1994}. With the inclusion of naps in our dataset, our analyses reveal compelling correlations and findings that aligned with prior sleep literature~\cite{Akerstedt1997,Borbely2016,Dijk1992}. Across all of our participants, 9.3\% of our data points included naps (mean duration: 73 mins). Of those cases, 62\% were automatically tagged and 38\% were manually tagged post-hoc. We have added these nap statistics in Section~\ref{sec:datasets-filtering}.
    \item \textbf{Device heterogeneity:} The app was deployed on both iOS and Android during this study. App interaction time is computed locally, so it is unaffected by network connectivity; however, rendering capabilities and other device specifications may have affected our calculation of app interaction time. Assuming that each participant kept using their own phone throughout the study, any device-specific idiosyncrasies would manifest in a consistent manner within their own data. Since we used generalized additive models that included \textit{UserID} as a random effect, device-specific effects are accounted for through the user-specific intercepts; we mention this fact in Section~\ref{sec:methods-rq2}. To the best of our knowledge, prior cross-device studies have not explicitly accounted for hardware/software differences when calculating event-driven measurements for this style of research~\cite{Vizer2009,Althoff2018}. In addition, we find biologically plausible and meaningful results that suggest that the data includes meaningful variation regardless of device-specific effects.
    \item \textbf{Variation in fees collected:} After further analysis based on R5's suggestion, we found that the fees were highly variable (\$250--\$1,750) in a non-normal manner. The fees are dependent upon the nature of the clients rather than the employees' performance. Therefore, we have decided that the amount of fees collected is an inappropriate job performance metric and exclude it from our analyses. We have justified this decision in Section~\ref{sec:datasets-job}.\\
\end{itemize}
Outside of these factors, we were unable to investigate the others for one of a few reasons: 
\begin{itemize}[leftmargin=.35in]
    \item Our data does not have sufficient variance to meaningfully analyze such questions (e.g., work hours, age, international travel)
    \item There is no objective way of measuring those data without adding potential sources of uncertainty (e.g., concussion, stress)
    \item Collecting those data would have required extra work from users (e.g., caffeine). To elaborate this point, we consider the fact that our app-based performance metric is completely passive to be one of the strengths of our work. Regularly logging information on factors like caffeine and nutrition would have placed additional burden on our study participants, which may have discouraged repeated app interaction.
\end{itemize}
In most cases, we have cited literature in our responses to R5 that discuss various factors and potential confounds in the context of our study. Due to paper length concerns by R4, we have only added a subset of these issues to our revised article. Section~\ref{sec:discussion-context} discusses the fact that data from additional sources could lead to more meaningful sleep-tracking results, which we believe covers many of these concerns. \\

\item \reviewcomment{Paper length: R4 thought the paper was too long (though R5 disagreed). I think the length was reasonable though it will be better to tighten up the intro and findings sections.}
We removed analyses involving the fees collected by salespeople due to the concerns expressed by R5; as mentioned earlier, the amount earned from each client is mainly driven by the nature of their case rather than the abilities of the salesperson themselves. Removing the use of fees collected in our analyses eliminated a couple of figures and table rows in our results section. We have also followed R4's suggestion by removing some text from the introduction and the results sections. Otherwise, we have addressed the reviewers' comments in our revised article while roughly maintaining the same paper length. \\
\end{enumerate}

==> revisions/2ae.tex <==
\subsection{2AE} % reject, low impact
We appreciate the critical feedback the reviewer has provided, and we believe that addressing their concerns has made our article much stronger. Please find our responses to the reviewer's individual comments below:

\label{sec:revisions-2ae}
\begin{enumerate}[labelsep=6mm,label=(2AE-\arabic*)]
\item \reviewcomment{I was disappointed that the data from the sleep sensor only included when users went to bed and woke up and not the quality of the sleep: it seems that the sensor used has now the capability of analyzing sleep quality but perhaps it was not the case when the user study was done?}
The reviewer raises the insightful point that a person's perception of their sleep quality is not always a function of the metrics recorded by the Emfit QS sensor. There is no unanimous definition of sleep quality from the sleep science community \cite{Harvey2008,Ravichandran2017}. We have deliberately used the phrase ``sleep behavior'' rather than ``sleep quality'' because sleep quality is not as well-defined as the metrics we leverage in our analyses. Therefore, we focus on correlations relative to the mattress sensor's objective metrics and leave the consideration of sleep quality to future work. In fact, we posit that job performance may be influenced by a person's perception of their own sleep quality, so our research may inform ways of defining sleep quality in the future. We address the limitations behind sleep quality in Section~\ref{sec:discussion-recommendations}.\\

\item \reviewcomment{I am not surprised that the results of the correlation with sleep duration are not there: being in bed does not mean sleeping or sleeping well.}
We agree that there is a nuance between ``time-in-bed'' and ``total sleep duration'' since people may not fall asleep as soon as they get into their bed. The Emfit QS mattress sensor reports both metrics, but we restricted our analyses to time-in-bed because it only requires accurate presence detection; total sleep duration requires accurate presence and sleep detection, thus adding an additional source of potential uncertainty. We have updated all mentions of total sleep duration to time-in-bed and updated the definition in Table~\ref{tab:metrics}. \\

Literature has shown that time-in-bed recorded from sleep diaries is highly correlated with total sleep duration~\cite{Rogers1993}. We calculated the Pearson correlation between time-in-bed and total sleep duration in our dataset and also found a strong correlation ($\rho=0.85, p<.001$). Furthermore, we re-ran our analyses with total sleep duration instead of time-in-bed and found comparable correlations in almost all cases. We mention that we tested both metrics in Section~\ref{sec:dataset-sleep}. \\

\item \reviewcomment{I am not sure we are learning much from this paper: there are few correlations reported and some claims are given about the effect of the app engagement on sleep over time which are not well justified.} 
We thank the reviewer for their candid feedback on the impact of our findings. We feel that the results reported in this article accurately reflect the subtle and complex relationships we analyzed. We posit that larger effect sizes are not necessarily expected in this setting. As a point of comparison, Althoff et al.~\cite{Althoff2017} found that hour-long differences in time-in-bed resulted in keystroke timing differences of a few milliseconds ($\sim$3.5\%). As R5 thoroughly comments in their review, the small performance impacts we see are partly due to the rich set of factors impacting sleep and performance. For instance, sleep behavior is known to be affected by ambient light~\cite{Kozaki2005}, caffeine intake~\cite{Landolt1995}, and diet~\cite{Halson2008}, while salesperson job performance is influenced by their on-job experience and the state of the economy. Still, we were able to uncover statistically significant results that aligned with expectations from sleep science~\cite{Akerstedt1997,Borbely2016,Dijk1992}. Therefore, we believe these findings are meaningful to the research community. \\

Given the valuable feedback from the reviews, we have adjusted our article so as not to overstate our results; nevertheless, we also do not want to undermine the importance of the novel insights we provide in the paper. We reemphasize their novelty below:
\begin{itemize}[leftmargin=.35in]
    \item \textbf{RQ.1:} Previous research on the relationship between sleep behavior and performance has typically involved low-level performance metrics (e.g., reaction time~\cite{Rajdev2013,Ramakrishnan2012}) or constructed scenarios (e.g., basketball practice~\cite{Mah2011}). To the best of our knowledge, we are the first researchers to compare both sleep behavior and job performance across careers and during participants' everyday living using an automatic sleep-tracking technology.
    \item \textbf{RQ.2 and RQ.3:} Prior work has used smartphone interactions to estimate high-level constructs like stress~\cite{Ferdous2015}, mood~\cite{Golder2011,Mehrotra2016}, academic performance~\cite{Wang2015}, inebriation~\cite{Bae2017,Mariakakis2018}, accident risk~\cite{Althoff2018}, and even sleep~\cite{Murnane2016,Althoff2017}. We build upon this literature by demonstrating that app interaction time aligns with models of sleep behavior as conveyed by operationalized sleep metrics from automatic sleep sensing. We then align app interaction time with job performance data to add to the coverage of aforementioned literature. 
    \item \textbf{RQ.4 (which we have reframed per suggestions by R5):} Prior work on automatic sleep sensing has focused on the accuracy of their underlying signal processing compared to a gold-standard (e.g., polysomnography, sleep diary)~\cite{Rahman2015,Min2014}. Sleep tracking is known to improve one's awareness of their sleep habits~\cite{Choe2011,Daskalova2016,Daskalova2018}; however, it is unclear if that awareness translates into improved sleep~\cite{Liang2016}. Our longitudinal dataset with an automatic sleep sensor provided us with the unique opportunity to explore this question. We demonstrated that improved sleep behavior was associated with the engagement with automatic sleep tracking. \\
\end{itemize}

\item \reviewcomment{I am also a bit skeptical by the use of app interaction features as an indicator of ``alertness'' or ``cognitive capacity''. There is very little substantiation that this could be true for such a simple app.}
To further motivate our use of mobile app usage as an indicator of cognition and performance, we have added additional examples of prior work in this space to Section~\ref{sec:related-interaction}~\cite{Mark2014,Pielot2015,Oulasvirta2012,Vizer2009,Mehrotra2016,Ferdous2015}. For example, Murnane et al.~\cite{Murnane2016} demonstrate that app usage patterns vary for individuals with different chronotypes and rhythms of alertness. Oulasvirta et al.~\cite{Oulasvirta2012} correlated frequent, short bursts of smartphone interaction with inattentiveness, and Vizer et al.~\cite{Vizer2009} used variation and drift in keystroke rate to infer stress. \\

Regarding the substantiation of our findings, prior work on sleep science supports our findings from the generalized additive model shown in Figure~\ref{fig:app-perf}. For example, our findings illustrate that users typically had slower interaction times immediately after waking up, which aligns with the chronobiological process of sleep inertia~\cite{Akerstedt1997}. We also found that interaction time decreased during the first six hours after wakeup and then increased again, which is consistent with the chronobiological process of homeostatic drive~\cite{Borbely2016}. These findings are consistent with chronobiological studies, and suggest that app interaction times include meaningful variation. \\

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/app-perf-time-sleep-history-full_population.pdf}
    \includegraphics[width=1.0\linewidth]{imgs/app-perf-time-sleep-debt.pdf}
    \vspace{-8mm}
    \caption{(Top row) The generalized additive model of interaction time against \revision{the local time in the user's time zone}, time since wake-up, and sleep history. 
    (Bottom row) A similar generalized additive model using sleep debt instead of sleep history. Standard errors are shown in both cases. Both models included random intercepts for each user.}
\end{figure}

\item \reviewcomment{The paper title refers very much to job performance; however, it seems that the novelty as presented in the paper is very much about app engagement effects more than job performance effects from sleep. Perhaps the work needs some repositioning.}
Thank you for the suggestion on the framing of our contribution. We appreciate the fact that our usage of app interaction time is exciting for the IMWUT community and are equally excited about the prospect of correlating sleep and job performance data through our dataset. 
We have reworded our title to the following: ``Sleep Behavior, Job Performance, and Their Indicators in Mobile App Usage'' to give the three components in our dataset equal weighting. \\
\end{enumerate}

==> revisions/r3.tex <==
\subsection{R3} % accept, significant impact
\label{sec:revisions-r3}
\begin{enumerate}[labelsep=6mm,label=(R3-\arabic*)]
\item \reviewcomment{This MS contributes a clear, logical exploration of the use of sensor and app data that can be used to identify performance costs from sleep habits. The sensor and app data are specifically designed to be things that one could imagine scraping from someone without increasing their burden, making the findings useful to those thinking about scalable solutions. The paper is rich with data and figures, allowing a nuanced analysis by the reader, but it is well organized and concise. This paper will be of value to those interested in sleep, performance, passive extraction of signal from ambient data, and the use of correlated data across home sensors and in-the-world phone data patterns.}
We thank the reviewer for this very positive feedback about the methods and implications of our study. 
The reviewer raises an important point that sleep quality and job performance are difficult to assess in a non-intrusive manner, and that doing so passively enables large-scale experiments on these topics. We also agree that the ability to align and merge data from many sources is an exciting opportunity for future research teams to do novel interdisciplinary work. The increasing ubiquity of sensors in everyday life creates new ways to non-intrusively measure activities and metrics that are relevant to daily life.

\end{enumerate}

==> revisions/r4.tex <==
\subsection{R4} % major revision, medium impact
\label{sec:revisions-r4}
We thank the reviewer for their comments on the framing and organization of our paper. Please find our responses to the reviewer's individual comments below:

\begin{enumerate}[labelsep=6mm,label=(R4-\arabic*)]
\item \reviewcomment{Overall, I thought the paper was too long so important information got lost or had to be really searched for. I have provided a few comments to potentially improve the quality of the paper.}
We thank the reviewer for their candid feedback on the length of our contribution. R3 called our initial paper ``well-organized and concise'', but the 1AE agrees that some trimming would make the contribution more succinct. Accordingly, we have removed some sentences from the introduction and evaluation. We have also removed some of the results and figures that were deemed to be uninformative to further consolidate our article. We have constantly paid attention to the length of our paper during this revision cycle, adding a minimal amount of text to address reviewer concerns while keeping our paper length commensurate to our contribution. After addressing all comments, the overall paper length has not changed significantly, and we believe that the length of this revised article is comparable to previous IMWUT articles with similar contributions. We address each specific suggestion on page length in more detail under their respective comments. \\

\item \reviewcomment{I like the research questions, however, you have results that accompany them in the introduction. I would save the results for the results section.}
To the best of our knowledge, typical IMWUT publications mention at least one result in their introduction in order to entice readers and tell them the significance of the work that they will be reading. Because we consider each research question to be equally important, we feel that reporting one important result per research question is necessary to fully convey our contribution. Presenting the results in the introduction also gives readers the ability to identify the research questions and key results early on so they can jump to sections that interest them the most. Nevertheless, we appreciate the fact that brevity is equally important and have thus removed some of the result details from the introduction. \\

\item \reviewcomment{Introduction is quite long, I am not sure that section 2 (related work) needs its own section. Much of section 2 can be condensed and combined with section 1.}
We agree that the introduction could be shorter and have removed a few sentences accordingly. However, we have kept the related work in a separate section since that is the standard organization for IMWUT articles. \\

\item \reviewcomment{For the mattress sensor, how did it compare with polysomnography? Ref 54 doesn't seem to have that information easily.}
Ranta et al.~\cite{Ranta2019} evaluated the Emfit QS sensor's heart rate and respiratory rate tracking ability against polysomnography, finding 98.7\% and 97.6\% agreement between the two. We have added two other references~\cite{Guerrero-Mora2012,Kortelainen2010} to our article that compared the Emfit QS sensor to polysomnography. Guerrero-Mora et al.~\cite{Guerrero-Mora2012} found that the Emfit QS sensor was 80\% accurate in detecting sleep/wake events when compared to expert annotations of polysomnography data. Kortelainen et al.~\cite{Kortelainen2010} further evaluated the Emfit QS sensor in regards to sleep stage classification against experts' annotation from polysomnography, again finding that the Emfit QS has 83\% sensitivity and specificity. \\

There is a nuance between ``time-in-bed'' and ``total sleep duration'' since people may not fall asleep as soon as they get into their bed. The Emfit QS mattress sensor reports both metrics, but we restricted our analyses to time-in-bed because it only requires accurate presence detection; total sleep duration requires accurate presence and sleep detection, thus adding an additional source of potential uncertainty. We have updated all mentions of total sleep duration to time-in-bed and updated the definition in Table~\ref{tab:metrics}. \\

Literature has shown that time-in-bed recorded from sleep diaries is highly correlated with total sleep duration~\cite{Rogers1993}. We calculated the Pearson correlation between time-in-bed and total sleep duration in our dataset and also found a strong correlation ($\rho=0.85, p<.001$). Furthermore, we re-ran our analyses with total sleep duration instead of time-in-bed and found comparable correlations in almost all cases. We mention that we tested both metrics in Section~\ref{sec:dataset-sleep}. \\

\item \reviewcomment{Methods has too many details. For example, each research question is explored again when they have already been introduced}
We list the research questions in the introduction to provide an overview of the points that will be addressed in the article and to highlight the results that will be found later on. We use Section~\ref{sec:methods} to explain the motivation behind the research questions, their inspiration from related work, and the analyses that were conducted to investigate them. These details require an understanding of the dataset, which is why we bring up the research questions again after Section~\ref{sec:dataset}. Putting the research questions in multiple places strikes a balance between making the takeaways of the paper clear to the reader (2AE, R4) and providing more details on our methods (R5). \\

\item \reviewcomment{RQ1 and RQ3 are related to the subpopulation of athletes and salespeople which make up only 12\% of the 274 participants. It is unclear if the other results (RQ2, and RQ4) are in the whole sample or the athletes and salespeople. It would make sense for results on the whole sample go first and then the subpopulation. N values as it relates to the RQs would help make this clear throughout the results.}
We have made a concerted effort to be explicit about our sample sizes (i.e., number of users and number of data points) throughout the paper. The sample sizes are now explicitly mentioned in the following sections and tables:
\begin{itemize}[leftmargin=.35in]
    \item Abstract
    \item Section~\ref{sec:intro}: Introduction
    \item Section~\ref{sec:datasets-job}: Job Performance Metrics
    \item Table~\ref{tab:dataset}: Dataset summary statistics
    \item Section~\ref{sec:methods}: Research Questions and Methods
    \item Section~\ref{sec:results}: Results
    \item Table~\ref{tab:spearman-corr-job-perf}: Analysis for RQ.1
\end{itemize} 

We appreciate the reviewer's useful suggestion for reordering the research questions; after some consideration, we have decided to keep our original question ordering as we feel that it better fits the narrative of the paper. Prior literature has hypothesized that sleep affects job performance (sleep $\rightarrow$ job performance). We introduce app interaction as a proxy measurement that fits between those two constructs, so we then show that sleep and app interaction are related (sleep $\leftrightarrow$ app interaction) and then that app interaction reflects job performance (app interaction $\leftrightarrow$ sleep). Therefore, our first question supports existing literature in sleep science, and then our next two questions build on top of more recent literature on technology interaction as an indicator of behavior. \\ 

\item \reviewcomment{What were the effect sizes? This is worth exploring as the correlation coefficients are low.}
Our original submission listed multiple effect sizes when our correlation coefficients were found to be statistically significant. To address questions that multiple reviewers had about the significance of the effect sizes, we expanded some of them by converting percentages to absolute quantities. We have enumerated the effect sizes presented in the article below for your convenience  (revisions to the article are in red):
\begin{itemize}[leftmargin=.35in]
    \item ``One hour of sleep loss the night before by the average salesperson resulted in 1.9\% decrease in the number of hires they were able to make. \revision{The average salesperson made 3.8 hires per workday and collected \$936 in fees per hire. Therefore, a 1.9\% decrease translates to a \$67 loss per day.}'' (Section~\ref{sec:rq1})
    \item ``The average athlete experienced a 2.0\% drop \revision{(1.3 points)} in their game grade when they lost one hour of sleep the night before.'' (Section~\ref{sec:rq1})
    \item ``A more severe, but not uncommon scenario of losing an hour of sleep every day for a week is equivalent to losing 4.75 hours of sleep yesterday or 11.2 hours of sleep one week ago. On average, this loss in sleep debt causes a 9.5\% \revision{(6.2 points)} reduction in game performance, and a 9\% \revision{(\$317)} reduction in hires for salespeople.'' (Section~\ref{sec:rq1})
    \item ``For one hour of sleep history improvement, the average athlete improved their game grade by 5.7\%.'' (Section~\ref{sec:rq1})
    \item ``Users who accumulated one less hour of sleep debt were 0.2 seconds faster each time they moved between app screens.'' (Section~\ref{sec:rq2})
    \item ``On average, interaction time increases by 0.4 seconds when sleep history improves from 6 to 8 hours, and interaction time increases by 0.5 seconds beyond the threshold of -5 sleep debt hours.'' (Section~\ref{sec:rq2})
    \item ``The effect size shows that athletes who were 10 seconds faster in their interaction time, on average had 5 more points higher game grades.'' (Section~\ref{sec:rq3})
    \item ``Participants who engaged with the app for 35 days on average slept 42 minutes longer, had 3.5 hours less sleep debt, and went to bed 48 minutes earlier, compared to less engaged users that opened the app on only 7 days. Participants who engaged with the app more often also exhibited more consistent bedtimes, with the standard deviation dropping from 1.4 hours to 1.2 hours.'' (Section~\ref{sec:rq4})
    \item ``Higher app engagement was consistently associated with an improvement in average time-in-bed within users, with an average increase in time-in-bed of about 15 minutes per night.'' (Section~\ref{sec:rq4})
\end{itemize}
~\\

\item \reviewcomment{``Since we found strong correlations between the cumulative sleep behavior metrics'' ... Typically strong correlations are defined as 0.6-0.8, 0.4-0.6 are moderate, 0.2-0.4 are weak, and 0.0-0.2 are very weak}
We thank the reviewer for making this point. We have revised this sentence to say that the correlation is ``statistically significant'' rather than just ``significant''. Although most of our statistically significant correlation coefficients would be considered ``weak'' according to this categorization, we posit that larger effect sizes are not necessarily expected in this setting. As a point of comparison, Althoff et al.~\cite{Althoff2017} found that hour-long differences in time-in-bed resulted in keystroke timing differences of only a few milliseconds ($\sim$3.5\%). As R5 thoroughly comments in their review, the small performance impacts we see are partly due to the rich set of factors impacting sleep and performance. For instance, sleep behavior is known to be affected by ambient light~\cite{Kozaki2005}, caffeine intake~\cite{Landolt1995}, and diet~\cite{Halson2008}, while salesperson job performance is influenced by their on-job experience and the state of the economy. Still, we were able to uncover statistically significant results that aligned with expectations from sleep science~\cite{Akerstedt1997,Borbely2016,Dijk1992}. \\

\item \reviewcomment{The figures look nice and are very clear. But the information gets lost with so many. I would hone in on your most important results as figures so the reader can focus on those.}
We appreciate that fact that you found the figures to be clear. We use the figures to illustrate effect sizes (RQ.1, RQ.3, RQ.4) and highlight the fact that our data aligns with the expectations of literature on circadian rhythms (RQ.2)~\cite{Akerstedt1997,Borbely2016,Dijk1992}. As R3 noted in their review, figures can provide a lot of information in a concise manner, particularly for readers who choose to skim through the paper. The figures also emphasize effect sizes that may have been otherwise lost in the text.\\

Nevertheless, we have taken this suggestion to heart as much as possible. We have also not included any of the additional figures that were requested by other reviewers, and we have also removed a subplot and table rows related to \textit{fees collected} due to concerns raised by R5. After further analysis, we found that the fees were highly variable from case-to-case (\$250--\$1,750), and the fees are dependent upon the nature of the clients rather than the employees' performance. Therefore, we have decided that the amount of fees collected is an inappropriate job performance metric and exclude it from our analyses. We have justified this decision in Section~\ref{sec:datasets-job}. \\
\end{enumerate}

==> revisions/r5.tex <==
\subsection{R5} % major revision, significant impact
\label{sec:revisions-r5}
We are impressed by the thoroughness of the reviewer's response and are greatly appreciative for their insights. One overarching response we would like to highlight is the fact that our app-based performance metric is completely passive. We believe this is one of the strengths of our work. Requiring participants to regularly log information on potential confounds would have placed additional burden on our study participants, which may have discouraged repeated app interaction. Even so, we have various responses to the different comments provided in the review and have made numerous changes in the article to alleviate some of these concerns.

\begin{enumerate}[labelsep=6mm,label=(R5-\arabic*)]
\item \reviewcomment{There is really nothing in the study to suggest that the N of the observed populations will be 15 and 19 until you get to Table 2.  While I understand this was done for presentation reasons, this really does a fairly large disservice for the broader community when this is done in papers, especially when big numbers are being tossed around (1.6 years, 30k nights of tracked sleep, 16k app interaction events).}
We have made a concerted effort to be explicit about our sample sizes (i.e., number of users and number of data points) throughout the paper. The sample sizes are explicitly mentioned in the following sections and tables:
\begin{itemize}[leftmargin=.35in]
    \item Abstract
    \item Section~\ref{sec:intro}: Introduction
    \item Section~\ref{sec:datasets-job}: Job Performance Metrics
    \item Table~\ref{tab:dataset}: Dataset summary statistics
    \item Section~\ref{sec:methods}: Research Questions and Methods
    \item Section~\ref{sec:results}: Results
    \item Table~\ref{tab:spearman-corr-job-perf}: Analysis for RQ.1 \\
\end{itemize}

\item \reviewcomment{Further, my natural inclination would be for a paper espousing mobile app usage to see mobile app usage / phone usage as a feature for evaluation rather than the app interactions being used as a proxy for PVT. The proxy for PVT is potentially neat and I think the potentially more beneficial aspect for the Ubicomp / passive sensing community as I would concur with the authors that doing a PVT can be jarring. I am a bit skeptical though that the methods used map nearly as well and I think comparing / contrasting the two population subsets would be strictly necessary versus the broader population of N=274.}
We agree with the reviewer that using app interaction time as a proxy for PVT, while a potentially beneficial application, would require an explicit comparison study. In this work, we did not intend for app interaction time to be a proxy for the PVT. The PVT strictly measures reaction time, while app interaction requires the user to process information on the screen; we have added a sentence where app interaction time is first introduced (Section~\ref{sec:datasets-app}) to clarify this fact. Instead, we assert that both the PVT and app interaction time relate to cognitive abilities that affect job performance, but the latter is easier to deploy in the wild. \\

Our analysis for RQ.2 (app interaction time vs. sleep behavior) was conducted for the broader population of N=274. Not only did we uncover statistically significant correlations between app interaction time and multiple raw sleep behavior metrics, but we also found that app interaction time was sensitive to circadian rhythms and sleep inertia~\cite{Akerstedt1997,Borbely2016,Dijk1992}. We compared and contrasted the two subpopulations in RQ.3 (app interaction time vs. job performance), finding that there is only a statistically significant correlation with app interaction time for the athletes. Our app interaction metric is partly related to reaction time, so the discrepancy between athletes and salespeople in this analysis may be because the athletes' day-to-day activities require rapid, precise reactions; the salespeople's activities, on the other hand, are typically more forgiving in the sense of psychomotor function. Another explanation could be that PFF includes contextual information, such as whether the opponent presented a favorable matchup during a game; the number of hires a salesperson can make in a given day is more dependent upon external factors (e.g., customer needs, health of the economy) We have added this interpretation of the results to Section~\ref{sec:rq3}. \\

\item \reviewcomment{The subtle point of sleep debt versus normalized sleep debt on Page 2 of RQ.1 needs to be have a bit more context.}
Thank you for indicating this potential point of confusion. When we shortened our introduction per the requests of R4 and the 1AE, we removed the sentence that mentioned normalized sleep debt. This term is now fully defined when it is first introduced in Section~\ref{sec:dataset-sleep}. \\

\item \reviewcomment{How much variation was there in terms of the hours worked by the salespeople? What hours did the salespeople work? Were they working strictly 9 to 5? Is there fatigue that plays a role for those working longer hours?}
The figures below show the distributions of the times at which people started (left) and ended (middle) each workday, as well as the daily work hours (right). Across all participants, 66\% workdays started between 7--9 AM, and 52\% ended between 4--6 PM.
Additionally, 67\% of the workdays lasted 6--8 hours, and less than 5\% of the workdays were longer than 9 hours. Given that a standard workday in the United States is 8 hours, we do not believe that exceptional fatigue played a significant role in these results. Although work hours were generally consistent across the salespeople, we normalized our data to account for whatever variance remained. \\

\begin{figure*}[h]
\centering
\includegraphics[width=.33\linewidth]{imgs/upright_starthour_histogram.pdf}
\includegraphics[width=.33\linewidth]{imgs/upright_endhour_histogram.pdf}
\includegraphics[width=.33\linewidth]{imgs/upright_workhours_histogram.pdf}
\caption{Histograms showing summary statistics for their (left) start time, (middle) end time, and (right) total work duration.}
\label{fig:histogram_workhours}
\end{figure*}

\item \reviewcomment{Does experience as well play a role in terms of years in the position?}
We agree that analyzing the effect of experience on job performance would yield a compelling analysis. Unfortunately, we did not have experience data for our participants in this study. We also did not have information about participants' work experience prior to their current position, which may be equally important. One statistic we were able to retrieve from the bankruptcy law firm consultancy is that 88\% of their employees have been at the company for less than 2 years. Getting statistics on the experience of the NFL players is complicated by the fact that the number of years they spend in the NFL does not always translate to gameplay. Some players may start every game for 5 seasons, while other may only play for a couple of snaps over the same duration. These issues make it difficult to perform a meaningful analysis for either subpopulation. \\

\item \reviewcomment{The nights of sleep tracked with job performance measures is a bit tricky. It would be helpful to list the number of evaluation points (esp. for athletes) in Table 2.}
We agree with the reviewer that this clarification is important. We have made a number of changes to Table~\ref{tab:dataset} to clarify the definition of each dataset summary statistic. For example, we have changed ``nights of tracked sleep with job performance measures'' to ``total unique days with both sleep-tracking and job performance measurements''. We have also added a new row that reports the number of tracked nights of sleep overall for each population. We repeat the most relevant sample size numbers in the first sentence of each subsection in Section~\ref{sec:results} (with the exception of RQ.4, where the sample sizes are included in Figure~\ref{fig:sleep-improvement}). \\

\item \reviewcomment{How much noise there in the PFF or variation amongst the experts?}
Details about PFF's ranking method can be found on an archived version of their website~\cite{ProFootballFocus2017}. Two experts individually assign a score from -2 to 2 with increments of 0.5 for each play, and then a third expert resolves any disagreements. Those per-play scores are summed together and then normalized to a grade between 0-100. The grades are reviewed by the Pro Coach Network, a collection of ex-players and coaches with NFL experience. Although there may be some disagreement between the first two experts, the discrepancy is likely no greater than 0.5 per play since they will at least agree on whether the play had a good or bad outcome. The third expert and the Pro Coach Network reviews also add stability in PFF scores. Because of this thorough process, we believe PFF is a rigorous and strong indicator of performance in the NFL. We have added more detail to our description of PFF's scoring procedure in Section~\ref{sec:datasets-job} and included the previously missing reference. \\

\item \reviewcomment{A bit more on sleep debt would be helpful in the introduction.}
We agree with the reviewer that more clarification on this terminology early on would be useful. We have modified the sentence in the introduction that uses the term ``sleep debt'' for the first time to explain that it is a cumulative metric of sleep loss. We leave the more complete definitions for later to avoid adding too much text (as suggested by R4). \\

\item \reviewcomment{I'm not sure that the NFL collects gold standard job performance data, the phrase in the intro seems to suggest that. You are using the PFF (not a bad choice) but it is not done by the NFL.}
We thank the reviewer for highlighting this mischaracterization of PFF scores. Instead of calling PFF a ``gold-standard'', we revised the text to say that PFF is ``widely accepted'' as a performance metric since it has been used in past academic literature \cite{Dodson2016,Provencher2018,Byanna2016}. We have also removed the statement that said that the NFL is responsible for calculating the PFF scores. \\

\item \reviewcomment{While the Althoff work points to interesting aspects, it feels a bit like there should be more validation of the interactions. In my mind, this is the more exciting part for the community and something that others can grab onto for future work. It gets some focus but not nearly enough in the paper versus the flashier sales / athlete focus.}
We thank the reviewer for their excitement about our use of mobile app usage as an indicator of job performance and sleep behavior. To further motivate our use of mobile app usage, we have added additional examples of prior work in this space~\cite{Mark2014,Pielot2015,Oulasvirta2012,Vizer2009,Mehrotra2016,Ferdous2015} (Section~\ref{sec:related-interaction}). For example, Murnane et al.~\cite{Murnane2016} demonstrate that app usage patterns vary for individuals with different chronotypes and rhythms of alertness. Oulasvirta et al.~\cite{Oulasvirta2012} correlated frequent, short bursts of smartphone interaction with inattentiveness, and Vizer et al.~\cite{Vizer2009} used variation and drift in keystroke rate to infer stress. \\

Regarding our own findings, the generalized additive model we generated in Section~\ref{sec:rq2} aligns with expectations from prior work. Our findings illustrate that users typically had slower interaction times immediately after waking up, which aligns with the chronobiological process of sleep inertia~\cite{Akerstedt1997}. We also found that interaction time decreased during the first six hours after wakeup and then increased again, which is consistent with the chronobiological process of homeostatic drive~\cite{Borbely2016}. \\

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/app-perf-time-sleep-history-full_population.pdf}
    \includegraphics[width=1.0\linewidth]{imgs/app-perf-time-sleep-debt.pdf}
    \vspace{-8mm}
    \caption{(Top row) The generalized additive model of interaction time against \revision{the local time in the user's time zone}, time since wake-up, and sleep history. 
    (Bottom row) A similar generalized additive model using sleep debt instead of sleep history. Standard errors are shown in both cases. Both models included random intercepts for each user.}
\end{figure}

We also thank the reviewer for pointing out that our potential overemphasis on the flashier sales/athlete focus. This observation was echoed by the other reviewers, particularly with the title. As such, we have changed the title to ``Sleep Behavior, Job Performance, and Their Indicators in Mobile App Usage''. This title does not mention the notion of athletes and salespeople in our dataset to avoid misleading readers into thinking that the entire dataset consists of those individuals, and it also gives equal weighting to the three components of our dataset. \\

\item \reviewcomment{The redaction for the sleep tracking mobile app (Page 5, footnotes 3 and 4) makes it hard to discern the accuracy of sleep and whether or not phone usage will impact sleep start / stop detection. Was the sleep tracking app done by the authors? It would seem so but some clarity would be helpful.}
We redacted the name of the sleep tracking app to preserve our anonymity as authors. The research in this submission comes from a collaboration with the company who developed the sleep-tracking app, but most of the authors were not directly involved in the creation of the app. To ensure there is no confusion regarding the mechanisms of sleep tracking, we would like to reiterate that the sleep metrics are only extracted from the Emfit QS sensor. The smartphone only provides an interface through which users can see their data. None of the authors had a hand in the development of the Emfit QS sensor. We believe that the involvement of the authors with the technologies in our study will be clear if and when the author list can be added to the article. \\

\item \reviewcomment{Was the app released for both Android and iOS? Are there potentially mobile device speed issues in terms of rendering? What if one has say an iPhone 6 versus say the newest Samsung Galaxy? Are there network effects (WiFi vs. cellular) that can also play a role or is everything cached locally?}
The app was deployed on both iOS and Android during this study. App interaction time is computed locally, so it is unaffected by network connectivity; however, the reviewer is correct in noting that rendering capabilities and other device specifications may have affected our calculation of app interaction time. Assuming that each participant kept using their own phone throughout the study, any device-specific idiosyncrasies would manifest in a consistent manner within their own data. Since we used generalized additive models that included \textit{UserID} as a random effect, device-specific effects become lumped into the user-specific intercepts; we mention this fact in Section~\ref{sec:methods-rq2}. To the best of our knowledge, prior cross-device studies have not explicitly accounted for hardware/software differences when calculating event-driven measurements for this style of research~\cite{Vizer2009,Althoff2018}. \\

\item \reviewcomment{Generally speaking, accelerometer / weight sensors tend to do pretty poorly discerning sleeping versus lying in bed watching TV / using your phone.}
We agree that there is a nuance between ``time-in-bed'' and ``total sleep duration'' since people may not fall asleep as soon as they get into their bed. The Emfit QS mattress sensor reports both metrics, but we restricted our analyses to time-in-bed because it only requires accurate presence detection; total sleep duration requires accurate presence and sleep detection, thus adding an additional source of potential uncertainty. We have updated all mentions of total sleep duration to time-in-bed and updated the definition in Table~\ref{tab:metrics}. \\

Literature has shown that time-in-bed recorded from sleep diaries is highly correlated with total sleep duration~\cite{Rogers1993}. We calculated the Pearson correlation between time-in-bed and total sleep duration in our dataset and also found a strong correlation ($\rho=0.85, p<.001$). Furthermore, we re-ran our analyses with total sleep duration instead of time-in-bed and found comparable correlations in almost all cases. We mention that we tested both metrics in Section~\ref{sec:dataset-sleep}. \\

\item \reviewcomment{Are there potential issues with regards to partners / family members lying in the bed as can occur with mattress-based systems?}
The Emfit QS sensor comes with instructions that explain how to install the sensor in situations when a bed is shared by multiple people (page 6 of \cite{Emfit2018}). The sensor can be placed so that it lies solely on the user's preferred side of the bed. The sensor has been designed to filter out smaller displacements in favor of larger ones caused by the user lying directly on top of the sensor. We have added this information to the revised article. \\

\item \reviewcomment{What about the impact of naps? Were those logged / recorded separately via the app?}
The time-in-bed metric we report includes naps that were either automatically tagged by the Emfit QS sensor or manually annotated post-hoc by the user if they were missed. We feel that it is important to include naps in our dataset because they contribute to sleep recovery, thus contributing to sleep debt/sleep history~\cite{Matsumoto1994}. With the inclusion of naps in our dataset, our analyses reveal compelling correlations and findings that align with prior sleep literature~\cite{Akerstedt1997,Borbely2016,Dijk1992}. Across all of our participants, 9.3\% of our data points included naps (mean duration: 73 mins). Of those cases, 62\% were automatically tagged and 38\% were manually tagged post-hoc. We have added these nap statistics in Section~\ref{sec:datasets-filtering}. \\

\item \reviewcomment{What was the general compliance for the salespeople and athletes? A table describing that compliance would be very helpful. The +/- for monitoring was pretty brutal on both of them, 46.33 +/- 37.45 and 133.1 +/- 89.92. That implies potentially a huge amount of imputation (that details which was buried deep / late in the paper). The imputation details (Page 16) are super important and should have been brought out when discussing the sensors themselves. As the standard deviation was on the order of half of the days observed, this could represent a huge amount of imputation. Further, given that it is imputing from nearby days, is that accurate? I would recommend testing this to see if this assumption holds generically across the participants.}

Thank you for bringing up this important point. The large standard deviations in Table~\ref{tab:dataset} imply to readers that compliance was low and lots of imputation was needed in our dataset. However, we believe that these numbers are a bit misleading in that regard. Compliance can be broken into two levels: organization engagement and participant compliance: \\

\textbf{Organization engagement:} Our dataset is the product of a collaboration with multiple organizations. To recruit the NFL players, for example, we were unable to engage with the entire league and thus had to form partnerships with individual teams. Although our data collection period lasted 1.5 years, the level of engagement we had with different organizations varied. The bankruptcy law firm consultancy was enrolled for 225 days, and the NFL teams were enrolled from 457--518 days. Across our entire population, participants were enrolled for 83--578 days. This aspect of our recruitment means that even if participants engaged with the sleep-tracking technology every day, there would still be large variance in the number of nights of tracked sleep as summarized in Table~\ref{tab:dataset}. \\

\textbf{Participant compliance:} As we stated in our article, participants were free to enroll and leave the study as they pleased. This means that some participants started later than others once their organization joined our study. Participants were also free to use the sleep-tracking technology however they wanted. This was done to reduce friction with our partnered organizations and to generate the most natural data possible. Table~\ref{tab:imputed_sleep} shows the fraction of sleep duration values that were imputed in the calculation of the sleep history metric. A full week of sleep data was available for calculating 46.9\% of the cumulative sleep metrics, meaning that no imputation was needed for them. Three or more nights were only missing in 12.7\% of the cumulative sleep metrics. More sleep history metrics required imputation for the athletes, likely because travel caused more missed tracked nights of sleep. \\

We agree that the matter of imputation should be highlighted much earlier in the paper and thank the reviewer for raising this issue. Our original article described the nature of our recruitment process in Section~\ref{sec:dataset-population} and our imputation procedure in Section~\ref{sec:dataset-sleep}. On top of this, we have removed the ``Observation Period'' row in Table~\ref{tab:dataset} to avoid misleading readers into thinking that enrollment was continuous. We provide the above reasoning in Section~\ref{sec:datasets-filtering} to describe why the standard deviations are so large in Table~\ref{tab:dataset}. We have also added statistics on the amount of imputation that was needed in Section~\ref{sec:datasets-filtering}. \\

% THIS TABLE IS FROM SLEEP DATA THAT WE HAVE INTERACTION DATA FOR (NO DOUBLE COUNTS)
\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c}
         Number of & Full & & \\
         Imputed Days & Population & Salespeople & Athletes \\
         \hline
         
         0 & 46.9\% & 49.2\% & 29.2\% \\
         1 & 24.6\% & 15.3\% & 45.3\% \\
         2 & 15.8\% & 13.6\% & 12.3\% \\
         3 & 8.6\% & 16.1\% & 8.2\% \\
         4 & 4.1\% & 5.9\% & 5.0\% 
         
    \end{tabular}
    \caption{Number of imputed days in sleep history calculation.}
    \label{tab:imputed_sleep}
\end{table}
% full_population
% num interactions data: 12183
% num night sleep: 5813 <-- imputations calculated over this.
% num_days
% 3.0     237     4.1\%
% 4.0     498     8.6\%
% 5.0     919     15.8\%
% 6.0    1430     24.6\%
% 7.0    2729     46.9\%
% sales
% num interactions data: 274
% num night sleep: 118 
% num_days
% 3.0    7    5.9\%
% 4.0    19   16.1\%
% 5.0    16   13.6\%
% 6.0    18   15.3\%
% 7.0    58   49.2\%
% athletics
% num interactions data: 704
% num night sleep: 342 
% num_days
% 3.0    17   5.0\%
% 4.0    28   8.2\%
% 5.0    42   12.3\%
% 6.0    155  45.3\%
% 7.0    100  29.2\%


\begin{figure*}[h]%
\centering
\subfigure[Nights of sleep tracked by salespeople]{%
\label{fig:first}%
\includegraphics[width=.4\linewidth]{imgs/upright_tracked_sleep_histogram.pdf}}%
\qquad
\subfigure[Nights of sleep tracked by NFL players]{%
\label{fig:second}%
\includegraphics[width=.4\linewidth]{imgs/nfl_tracked_sleep_histogram.pdf}}%
\caption{Histogram of nights of sleep tracked for salespeople and athletes}
\label{fig:histogram_sleep_tracked}
\end{figure*}

We agree that imputing with a short-term average will not always be perfect since participants may catch up on sleep when they are deprived the previous day or vice-versa. We have tested the validity of using imputing with the short-term average by computing the standard deviation of time-in-bed values whenever sleep debt was calculated without imputation. We found that the standard deviation was 1 hour and 10 minutes; this shows that there was not significant variance within a week, justifying the use of a short-term average. We also prefer average imputation for its interpretability, as advanced methods like regression-based or covariate-based imputation could lead to their own peculiarities. \\

\item \reviewcomment{Using the mobile phone agent as a sleep detection mechanism as a backup (see for instance StudentLife) might be a good starting point but keeping the app alive in the background can be a bear.}
This would be an excellent follow-up study for the IMWUT community. There have been numerous efforts in sleep sensing using technologies like smartphones and smartwatches~\cite{Ko2015,Min2014,Rahman2015,Byanna2016}, and they have achieved promising results. We actually investigated the inclusion of a sleep detection app that leveraged the accelerometer to sense bed motion. At the time, we found that the mobile app generally overestimated time-in-bed by 1-2 hours. These errors, combined with the burden of continuous battery drain to detect sleep events, led us to not feel comfortable with the introduction of an additional source of uncertainty. \\

\item \reviewcomment{Were any participants filtered out?}
Participants were filtered out of each analysis whenever they did not have the data necessary to answer that question. In RQ.1, for example, participants were excluded when they did not have at least one job performance metric with corresponding night of sleep-tracking. There were several participants who tracked their sleep consistently but were filtered out because they did not have any performance data. These cases occurred when athletes did not play in a particular game or when salespeople went on-leave. Conversely, participants who never tracked their sleep but constantly played in the games or showed up to work were also filtered out. The study populations shown in Table~\ref{tab:dataset} ($N=19$ for NFL players and $N=15$ for salespeople) were calculated after participants were filtered out using our conservative criteria. \\

\item \reviewcomment{What was the number of nights tracked versus performance observations? As noted above, it is difficult to figure out how many performance measures that you have for each subset. While N=118 nights is helpful (similarly N=171 nights for the athletes), the athletes have a much smaller set of actual performance points?}
We have clarified the data in Table~\ref{tab:dataset} to better explain our sample sizes. The N=118 and N=171 refer to the number of unique job performance measurements that had a corresponding night of tracked sleep. In other words, we ignored job performance measurements whenever there was no sleep tracking data to go with them. \\

\item \reviewcomment{For the athletes, were there impacts of day games versus night games (Monday / Thursday night football versus say a Sunday afternoon game)? Did the distance of the travel and potential time zone shift matter? Were any of the athletes involved in the international games that occurred during the study window?}
We agree with the reviewer that these would be interesting questions for us to investigate with our dataset. Regarding the start time of the NFL games, we do not have enough variation in our dataset to meaningfully compare the different situations. There is typically only one Thursday game and one Monday game per week in the NFL, and only a few teams participated in our study. There are also only a few international games each season, and none of our participating teams travelled internationally. \\

Regarding the questions of travel distance and time zone changes, prior work has demonstrated that sleep behavior is not significantly affected by interstate travel~\cite{Richmond2007}. Literature examining the effect of travel on gameday performance has been less conclusive. Jehue et al.~\cite{Jehue1993} found that NFL teams on the West coast perform poorly when travelling across to the East coast for day games, but they have a distinct advantage on night games regardless of whether they are home or away. We briefly discuss these papers in Section~\ref{sec:discussion-context}. We also want to take this opportunity to emphasize that users were free to use the Emfit QS as they pleased. This means that participants were not required to carry the mattress sensor with them when they traveled, but could have if they chose to do so. We emphasize this point in Section~\ref{sec:dataset-population}. Within our NFL population, 7 of the 19 players took the Emfit QS with them at least once, and a time zone change only occurred during 1.2\% of our sleep events in our dataset. Therefore, travel had at most a minimal effect on our analyses. \\

\item \reviewcomment{For any of the athletes, could there be impacts by virtue of pain medication on app interaction? What about injuries? Could there be impacts on concussive effects?}
Although injuries are often publicly disclosed, injury reports are not always honest given the incentive for teams to keep their plans hidden from their opponents. Furthermore, prior work has not found a significant relationship between sleep and injury~\cite{Dennis2016}. Regarding concussions in particular, there is recent literature suggesting links between concussions and impaired cognitive function, yet there is no definitive method for diagnosing concussions. Studies estimate that almost 50\% of concussions go undiagnosed~\cite{Harmon2013}; this fact complicates the inclusion of a concussion variable in our dataset. We hope that our use of mobile app usage as a scalable indicator of sleep behavior and job performance could enable researchers to investigate hypotheses like these in the future. At this time, they are out of the scope of this work. \\

\item \reviewcomment{The lack of age data also seems like it could be important.}
We thank the reviewer for this suggestion. We did not collect age data from our participants; however, we are able to extract summary statistics on the ages of our subpopulations from their organizations. Within the bankruptcy law firm consultancy, 71\% of the employees were millenials~\cite{GreatPlaceToWork2017}. Within the NFL, most players are between 23-27 years old~\cite{Gertz2017}. There is no such source of age information for the other sleep-tracking app users. However, a study by Pew Research Center found that of the older adults who engage in self-tracking, only 2\% use computer programs and 1\% use mobile tools. We suspect that most of our participants are relatively young since self-tracking in our study required both a mobile app and a mattress sensor. \\

Given the limited age variance in our subpopulations, we expect that the results are fairly robust to this limited variation. Literature has shown that when statistically significant differences in sleep behavior are found across age groups, they are mainly found across large age differences of over 20 years~\cite{Yoon2003,Dijk1999,Feinberg1974}. Since we believe most of our participants were young adults, we believe that we would not have enough variance in our data to effectively answer this question and leave it to future work. We cite the aforementioned papers on the relationship between sleep and age in Section~\ref{sec:discussion-context}. \\

\item \reviewcomment{The normalized hours does concern me for the number of hires / attorney fees. Are the attorney fees the same? How much variation is there once normalized across individuals? Are their seasonal variations?}
We appreciate this feedback. We re-analyzed the distribution of fees amounts and found that they greatly vary from client-to-client (25$^{\text{th}}$-percentile = \$270, 75$^{\text{th}}$-percentile = \$1,760). Because the mapping between clients and salespeople is arbitrary, we recognize that fees do not properly reflect an employee's performance. As such, we have decided to remove fees collected as a job performance metric in our dataset. We describe this limitation in Section~\ref{sec:datasets-job} and focus our analyses on \textit{number of hires} throughout the paper. \\

We also discussed normalization at great length before our original submission. Had we not normalized number of hires, our representation of job performance would have favored people whose schedules allow them to work longer hours. By normalizing the metrics, we effectively study the salespeople's \textit{efficiency} at their jobs. In other words, we look more favorably upon a person who makes 4 hires in 4 hours than a person who makes 4 hires in 10 hours. This is similar to how PFF grades are made. PFF does not penalize players for not being on the field, but rather strictly grades players on their on-field performance. We believe that normalizing the salespeople's job performance is needed to make meaningful comparisons between the two subpopulations. \\

\item \reviewcomment{What about impacts of caffeine (coffee, soda) on performance? What about nutrition, meals?}
We agree with the reviewer that all of these factors impact sleep. Section~\ref{sec:discussion-context} already mentioned caffeine~\cite{Landolt1995} as a potential confound in our study, and we have added a citation regarding nutrition~\cite{Halson2008}. Researchers are currently exploring ways of automatically helping people track their diet~\cite{Bruno2017,Ye2016,Bettadapura2015}, which we envision will lead to a compelling avenue for future work. \\

\item \reviewcomment{For the athletes, what about the impact of the time of practice on app interaction performance?}
We did not look at this potential dynamic because prior work has found no relationship between exercise and memory consolidation/reaction time~\cite{Bosch2017}, the two factors that relate to our app interaction metric. However, we agree that this is an interesting aspect that could be explored in future work. \\

\item \reviewcomment{Are there performance metrics for the broader N=274? How do these two population subsets compare to that broader population?}
Our dataset is the product of partnerships with multiple organizations that had employees participate in our study. The analyses we present regarding job performance involve organizations that had job performance metrics available on at least a weekly basis. Therefore, we are able to compare the two subpopulations in RQ.1 and RQ.3, but we are unable to include the broader population in these analyses. The other research questions (RQ.2 and RQ.4), did not require job performance data, so they were conducted on the broader study population (N$=$274). We feel that comparing the subpopulations within the broader population in these questions would not produce insights that will generalize beyond those subpopulations, so we believe these will not supplement our contribution. \\

\item \reviewcomment{Is 2\% significant in terms of the number of hires? With N=15, that just seems tough to justify.}
Throughout our paper, we only computed effect sizes when statistically significant (p$<.05$); this was the case for when we computed the 1.9\% decrease in the number of hires the salespeople were able to make. This question could also be about the significance of the effect size's magnitude. The average salesperson made 3.8 hires per day and collected \$936 in fees per hire. Therefore, a 1.9\% decrease translates to a loss of \$67 per day. We went through a similar calculation to find that a 2\% decrease in PFF translates to a 1.3-point drop. We have added both of these calculations in Section~\ref{sec:rq1} to provide more context for our results. Although these differences may appear small to some readers, they can accumulate in many different ways:
\begin{enumerate}
    \item[(1)] Across multiple people on the same team
    \item[(2)] Across multiple nights with sleep loss
    \item[(3)] Over longer durations of sleep loss within the same night
\end{enumerate}
For example, salespeople who lost an hour hour of sleep every day for an entire week experienced a 9\% decrease in hires on average. \\

\item \reviewcomment{Did you control for chronotype?}
Bedtime, wake time, and local time are all metrics that capture chronotype to some extent in our generalized additive models for analyzing RQ.2. Using these metrics as a proxy assumes that a person's \textit{observed} chronotype according to their sleep behavior is equivalent to their \textit{true} chronotype; in other words, it assumes that an ``early riser'' typically wakes up in the morning and a ``night owl'' tends to stay up late. Although this is not always true, past researchers have also made this assumption and produced results from their data that align with the community's understanding of sleep behavior and chronotyping~\cite{Roepke2010,Althoff2017}. Furthemore, we explored correlations using these metrics and did not see any statistically significant correlations during our analyses. \\

\item \reviewcomment{For Figure 5, what about the base timezone versus the local time? Is localtime in terms of the base timezone or where the individual is currently at?}
Local time in Figure~\ref{fig:app-perf} is based on where the individual was when they fell asleep that night. We have clarified this in the figure's caption. \\

\item \reviewcomment{Is it really that surprising that folks participating in a sleep study improved their sleep? Maybe if this was done on the entire N=274, that might have a bit more interest.}
We thank the reviewer for bringing up this point for clarification. The analyses for RQ.4 were conducted on the entire study population (N=274). The sample size has been explicitly restated in the revised article. Regarding the novelty of our finding that participants actually improved their sleep, we argue that the link between engagement with automatic sleep-tracking technology and sleep improvement has not been shown in prior work. Prior work on automatic sleep sensing has focused on the accuracy of their underlying signal processing compared to a gold-standard (e.g., polysomnography, sleep diary)~\cite{Rahman2015,Min2014}. Sleep tracking is known to improve one's awareness of their sleep habits~\cite{Choe2011,Daskalova2016,Daskalova2018}; however, it is unclear if that awareness translates into improved sleep~\cite{Liang2016}. Since we found that participants improved their sleep over time and that sleep behavior was correlated with job performance, our findings suggest that sleep improvement can lead to an improvement in job performance. To make this contribution more clear, we have rephrase RQ.4 to ``Is engagement with automatic sleep-tracking technology associated with improved sleep behavior?''. We also better motivate for RQ.4 in the abstract, introduction, and Section~\ref{sec:methods-rq4}. \\

\item \reviewcomment{There is some thinking that apps capturing sleep and sharing sleep debt can contribute to anxiety / stress.}
Prior literature has suggested that self-tracking can cause stress when users generate broken mental models about the quantity they are tracking~\cite{Ravichandran2017}, and stress is known to negatively impact sleep behavior~\cite{Sadeh2004,Akerstedt2006}. Had that effect been prominent in our dataset, increased app usage would have led to worsening sleep over time; however, our analysis in RQ.4 demonstrated improvements in sleep over time. Measuring stress would have added a subjective metric into our dataset, thereby raising new concerns in our analyses. Although we recognize that stress still plays a major role in all of the data that we measured (sleep, job performance, and app interaction), we leave such an exploration to future work in the interest of space. \\

\item \reviewcomment{Were there personality metrics captured? I don't think you can argue RQ.4 without that. Otherwise, how do I know that the app is bringing me along / helping me to sleep more / better sleep debt or am I simply conscientious and being good about using the app?  With the limited number, that gets tough to really tease that out as well. Without controlling for conscientiousness or other factors, it is decidedly unclear whether or not RQ.4 can be meaningfully answered?}
Unfortunately, we did not collect personality metrics in our dataset. Personality metrics certainly play an important role whenever one seeks to explain why behavior change occurred for a given health-intervention technology. There are many psychological frameworks that researchers have developed to explain how personality plays a role in people's health-related decision-making~\cite{Taylor2006,Ajzen1998}, including the Health Belief Model~\cite{Hochbaum1958,Janz1984}, the Theory of Planned Behavior~\cite{fishbein1967attitude}, and the Transtheoretical Model~\cite{prochaska1984transtheoretical}. Questions about the underlying mechanisms of behavior change for our particular sleep-tracking tools are interesting, but they are out of the scope of our revised RQ.4. Although we are unable to explain every detail for \textit{why} sleep behavior improvement occurs, we argue that the fact that improvement even happened in the first place has not been shown in the context of an automatic sleep sensor. \\

\item \reviewcomment{What about the staying power of the engagement? Do they revert back outside of that 5 week period?}
We repeated the analysis in the second half of RQ.4 for different time-spans ranging from 3 to 7 weeks and the results were similar in all cases. Beyond 7 weeks, the percentage of participants who were still enrolled in the study fell to 35\% (Figure~\ref{fig:histogram_enrollment}). We chose to compare the effects of app engagement across a 5-week period because nearly 50\% of the participants were still enrolled by then.  \\ 

\begin{figure*}[h]
\centering
\includegraphics[width=.5\linewidth]{imgs/enrollment_duration_histogram.pdf}
\caption{Histogram showing the enrollment duration of the participants.}
\label{fig:histogram_enrollment}
\end{figure*}

\item \reviewcomment{Does app usage and knowing sleep debt encourage those with a larger sleep debt to go to bed earlier at the next opportunity?}
We agree with the reviewer that the feedback cycle between the user and their app presents an interesting opportunity for future work. Using our dataset, it is difficult to assess whether users who saw their sleep debt adjusted their sleep schedule at the next opportunity for two reasons: (1) Some users may have wanted to adjust their sleep schedule, but could not due to other restrictions. Conversely, some users may have been forced to change their schedule due to work demands or other factors in their life. Teasing apart this nuance would have required asking the user why they were changing their sleep schedule; and (2) users may not have decided to change their sleep schedule after seeing a high sleep debt value for the first time; instead, they may have waited some time before making a decision or acting on a particular value. Therefore, directly analyzing user's immediate responses to sleep debt values may miss out on cases when the app led to delayed sleep schedule changes. \\

Meaningfully answering this question would require an entirely new protocol that is out of the scope of this work. Nevertheless, we are able to show in our analyses that users who engaged with the app for 35 days on average went to bed 48 minutes earlier compared to less engaged users who only engaged with the app for 7 days (RQ.4). Although we cannot ascertain that changes happened immediately after users first saw their sleep debt value, we are able to demonstrate that schedule changes did occur with increased app engagement. \\

\item \reviewcomment{With the filtering for RQ.4, how many individuals did that filter? Looking at the large variations in compliance, that looks a bit worrisome if we were starting with N=15 and N=19 pre-filtering.}
We thank the reviewer for raising this point. Unlike the analyses that require both sleep and job performance metrics to be linked, this analysis requires app interaction and sleep, which was available for the entire study population ($N=274$); we have clarified this point of confusion in the text. For the second analysis in RQ.4 where we examine time-in-bed improvement (Figure~\ref{fig:sleep-improvement}), the number of users involved in each graph depends on their level of engagement. For each $D$, we filtered out users who has less than $D/2$ days of tracked sleep. The number of participants involved in each plot is now included along the top of Figure~\ref{fig:sleep-improvement}. \\

\item \reviewcomment{Did you look at weekday versus weekend effects on sleep and recovery? Did individuals work weekends?}
We did not look at the effects between weekdays vs. weekends. Previous research has already examined this relationship in great detail, uncovering numerous confounds like chronotype and age~\cite{Paine2016,Roepke2010}; however, this literature typically reframes the comparison between ``weekdays and weekends'' to one between ``scheduled and free days''. This is an important distinction for our dataset because different jobs require different schedules. Some of the salespeople in our dataset occasionally worked on weekends. The NFL players typically played on Sundays (for which PFF grades are available), but they also practiced on other days during the week depending on their travel and next game (for which PFF grades do not exist). Data collection also happened during the players' offseason, which entails an entirely different schedule for the players. Even the other participants in our dataset had jobs with various schedules that may not have adhered to typical weekday/weekend splits. Controlling for weekdays and weekends would have led to ambiguous data split, so we believe this question warrants a dedicated investigation in future work. We would also like to note that our most significant findings involved cumulative sleep metrics. When calculating these metrics, prior work has not distinguished between weekdays and weekends~\cite{Kitamura2016}. \\

\item \reviewcomment{It is hard to know if the app interactions can replace / be a better PVT as it is unclear whether these analyses are only on athletes / salespeople or done on the full study population. If it was only on the athletes / salespeople, it seems like a missed opportunity.}
We thank you for raising this point of confusion. The analyses for RQ.2 (sleep vs. app-based performance) were conducted with the full study population ($N$=274). We were only limited to the athlete and salesperson subpopulations when the analyses required job performance data. We have clarified this matter in Sections~\ref{sec:methods-rq3} and \ref{sec:rq3}. \\

\item \reviewcomment{Is data logged locally or is the sensor cloud used to get data?}
Both the sensor data from the Emfit QS and the interaction time from the app are uploaded to the cloud. Aggregated Emfit QS data is available to users through the app using an API, but the interaction time is only available to researchers. App interaction time is calculated locally on participants' smartphones, so it is not affected by network connectivity in any way. \\

\item \reviewcomment{There's actually a fairly large field about athletics and sleep and RT, and the Army does a lot (e.g., Balkin).}
We thank the reviewer for directing us to additional literature on the relationship between sleep and performance. We have cited four additional articles in Section~\ref{sec:related-sleepperformance} based on this suggestion. Belenky et al.~\cite{Belenky2003} (with Balkin) provide another study demonstrating the relationship between PVT performance and sleep. Killgore et al.~\cite{Killgore2006,Killgore2008} (with Balkin) demonstrate the relationship between total sleep deprivation and outcomes like emotional intelligence, constructive thinking, and decision-making during a gambling task. Finally, Watson~\cite{Watson2017} produced a survey paper on how sleep affects athletic performance. The paper we had cited on this topic by Mah et al.~\cite{Mah2011} makes up part of that survey. Our paper adds to this existing literature by (a) examining job performance metrics from different populations and (b) proposing the use of app interaction time as an indicator of job performance and sleep behavior. \\
\end{enumerate}

==> revisions/revisions.tex <==
\section{Review Responses}
We would like to thank the reviewers for reading the paper in detail and providing valuable, constructive feedback on our work.
We have used this revision cycle as an opportunity to significantly improve our article.
The most significant changes we have made are the following:
\begin{itemize}
    \item Reframed the title, abstract, and introduction to be more balanced in how the different components of our dataset are presented,
    \item Reported sample size numbers throughout the article,
    \item Provided more justification for the use of the mattress sensor and app interaction indicator,
    \item Removed \textit{fees collected} as an indicator of job performance,
    \item Reworded RQ.4 to more properly convey that piece of our contribution, and
    \item Added additional commentary on potential confounds.
\end{itemize}
We believe that our article provides thought-provoking and novel insights into the relationship between sleep, job performance, and mobile app usage, paving the way for future studies in this space.
For instance, we identify correlations between sleep behavior and real-life job performance, which has only been shown through in-lab or controlled cases in previous work.
We also demonstrate that passively captured app interaction metrics can serve as a useful indicator for some job performance and sleep measures.
Finally, it is widely accepted that self-tracking increases awareness about sleep; however, we show that increased engagement with automatic sleep-tracking technology is correlated with sleep improvement.

In the following pages, we have provided detailed responses to each of the suggestions, concerns, and questions raised by the reviewers.
The reviewers' comments are in boxes, and our responses to each comment follow.
Changes within the revised article itself are marked in red text.
In a few cases, reviewer remarks are grouped to avoid redundancy or reordered to cluster similar topics.
Our responses are structured as follows:
\begin{itemize}
\item Responses to 1AE: Page~\pageref{sec:revisions-1ae}
\item Responses to 2AE: Page~\pageref{sec:revisions-2ae}
\item Responses to R3: Page~\pageref{sec:revisions-r3}
\item Responses to R4: Page~\pageref{sec:revisions-r4}
\item Responses to R5: Page~\pageref{sec:revisions-r5}
\end{itemize}

\input{revisions/1ae.tex}
\input{revisions/2ae.tex}
\input{revisions/r3.tex}
\input{revisions/r4.tex}
\input{revisions/r5.tex}
